What is my data worth? From data properties to data value

Data today fuels both the economy and advances in machine learning and AI. All aspects of decision making, at the personal and enterprise level and in governments are increasingly data-driven. In this context, however, there are still some fundamental questions that remain unanswered with respect to data. \textit{What is meant by data value? How can it be quantified, in a general sense?}. The "value" of data is not understood quantitatively until it is used in an application and output is evaluated, and hence currently it is not possible to assess the value of large amounts of data that companies hold, categorically. Further, there is overall consensus that good data is important for any analysis but there is no independent definition of what constitutes good data. In our paper we try to address these gaps in the valuation of data and present a framework for users who wish to assess the value of data in a categorical manner. Our approach is to view the data as composed of various attributes or characteristics, which we refer to as facets, and which in turn comprise many sub-facets. We define the notion of values that each sub-facet may take, and provide a seed scoring mechanism for the different values. The person assessing the data is required to fill in the values of the various sub-facets that are relevant for the data set under consideration, through a questionnaire that attempts to list them exhaustively. Based on the scores assigned for each set of values, the data set can now be quantified in terms of its properties. This provides a basis for the comparison of the relative merits of two or more data sets in a structured manner, independent of context. The presence of context adds additional information that improves the quantification of the data value.

==> dataproperties.tex <==
\section{Deriving Data Value}
\label{properties}

We first enumerate a set of data facets that are relevant for assessing the data value of a data set in general. Each facet may in turn contain various sub-facets, based on the values of which we effectively evaluate the data. Each sub-facet could take a range of values, which may be binary, categorical or numeric. In this context, we would like to start our analysis by answering  the following questions, in order to get a relative valuation for the data sets.
\begin{enumerate}
    \item What are the various facets that could typically apply to a data set?
    \item Given a specific data set, and a set of data facets, is it possible to assess whether the facet is relevant for the data set? If yes, which are the sub-facets that are relevant? More specifically, is it an aspect of interest to the current owner or to a potential buyer, or to both parties? How much of the assessment can be done without context?
    \item Given the possible values that could be associated with each sub-facet, how do we define an ordinal ranking of the values independent of any end-application?
    \item For any data set in general, is it possible to define a way to compute or determine the value of the various sub-facets?
\end{enumerate}
The above are some of the questions that we will try to answer in this section. These will lead us to the next step of comparing two data sets, defined across the same set of facets.


\subsection{Detailed properties}
%A data set has characteristics that are intrinsic to the data set, which hold across the various ways in which the data set may be used, and characteristics that are extrinsic to it, where the value of the characteristic may vary with the use to which it is put. For instance, the structure of the data set, or the size, is an intrinsic characteristic, while the suitability of the data for learning a specific model is an extrinsic characteristic. We group the various characteristics under the different facets, and note that sometimes there is no sharp boundary separating the various characteristics. Further, some of the characteristics take values that are mutually exclusive, while others are not.
%\label{detailedproperties}
In the following, each box captures a top-level description of the sub-facets and a set of questions that relate to that specific facet. These terms may be defined differently across different usage scenarios; we use the definition that we consider most relevant in the context of data value assessment. Each question has a set of possible values, from which the respondent selects the value applicable for that data set. Each value is assigned a score, based on common preferences. The combined scoring across all the facets as defined in equation~\ref{eqn:dv} then yields a quantification of data value under these set of assumptions, which may be used for comparing with other data sets under the same set of assumptions, or for further fine-tuning when more context is available. Note that in the following, where the question has a binary response, a 'Y' or a 'N', the score is 1 for a 'Y' and 0 for a 'N' unless indicated otherwise. Further, a 'Dont know' option is possible for many questions, and this has not been explicitly shown here; when selected, it would have a score of 0.

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
      \multicolumn{3}{|c|}{ \parbox{3in}{Structured data is any data that has well defined boundaries, in the form as it is, and that can be used to identify data points, fields and instances. 

Unstructured data is data which, in the form given, does not have well defined boundaries to identify  data points  or instances. Examples include  binary data, blobs of text, video, audio and image files.

Semi-structured data is any data which in the given form has a structure, but where the content within the boundaries could contain unstructured data. Examples are XML and HTML documents.}}\\
\hline
       \parbox{1in}{What is the data structure?} &\parbox{1in}{Structured,Semi-structured,Unstructured} &
       \parbox{1in}{1.0, 0.5, and 0.25}\\
       \hline
    \end{tabular}
    \caption*{Data Layout}
    \label{tab:my_label}
\end{table}

\begin{mybox} {Data Layout (Structured/semi-structured/unstructured data)}

Structured data is any data that has well defined boundaries, in the form as it is, and that can be used to identify data points, fields and instances. 

Unstructured data is data which, in the form given, does not have well defined boundaries to identify  data points  or instances. Examples include  binary data, blobs of text, video, audio and image files.

Semi-structured data is any data which in the given form has a structure, but where the content within the boundaries could contain unstructured data. Examples are XML and HTML documents.\\
Information on structural aspect of the data:\\
a) What is the data structure? \mbox{\ooalign{Structured}}/\mbox{\ooalign{Semi-structured}}/\mbox{\ooalign{Unstructured}}\\ The respective scores for the above values would be 1.0, 0.5, and 0.25
%Is the data Unstructured?\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
%Is the data Semi-Structured?\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\

\end{mybox}



\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
      \multicolumn{3}{|c|}{ \parbox{3in}{In general we would state that more recent data is better than less recent data. Further, some data gets outdated more rapidly than others, and hence in general, if the data is relevant for a longer period, it is more useful.}}\\
\hline
       \parbox{1in}{How current is the data?} &\parbox{1in}{Latest/Recent/Old/Not Applicable} &
       \parbox{1in}{1, 0.75, 0.25, 0}\\
       
       
       \hline
    \end{tabular}
    \caption*{Data Age}
    \label{tab:my_label}
\end{table}


\begin{mybox} {Data age}
In general we would state that more recent data is better than less recent data. Further, some data gets outdated more rapidly than others, and hence in general, if the data is relevant for a longer period, it is more useful.\\
a) How current is the data?\\
~\mbox{\ooalign{Latest}}/\mbox{\ooalign{Recent}}/\mbox{\ooalign{Old}}/\mbox{\ooalign{Not applicable}}\\
Score: 1, 0.75, 0.25, 0 respectively.
b) Does the data become less useful with age? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Score: 0 and 1 respectively\\
c) Does the data gain value with age?
\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}} \\
d) Is there a known later instance of the data? \mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Score: 0 and 1 respectively\\
e) How frequently does the data get outdated/updated?
\mbox{\ooalign{Daily}}/\mbox{\ooalign{Weekly}}/\mbox{\ooalign{Monthly}}/\mbox{\ooalign{Yearly}}/\mbox{\ooalign{Not applicable}}/\mbox{\ooalign{Dont know}}\\
Score: 0.25, 0.5,0.75, 1.0, 0 and 0 respectively
\end{mybox}

\begin{mybox} {Data Volume}
This is the size of the data set, in KB,MB or other relevant unit, and would have a bearing on the storage and processing costs. Modulo a certain upper bound, more data is generally better than less data.\\
a) What is the data size?\\
\mbox{\ooalign{$size<$500MB;}}\mbox{\ooalign{500MB~\leq~$size$~< 10G;}}\\
~\mbox{\ooalign{10G~$<size$~\leq~100G;}}~\mbox{\ooalign{$size>$ 100G}}\\
Score: 0.5, 0.75, 1.0 and 0.5 respectively.
\end{mybox}
%\begin{mybox} {Data Type}
%Data type is defined by the values it can take, or the operations (mathematical, relational or logical) that can be performed on it. \\
%is a classification that specifies which type of value a variable has and what type of  operations can be applied to it without causing an error.
%Questions in this category:\\
%What is the type of Data?\\
%\mbox{\ooalign{string}}/\mbox{\ooalign{binary}}/\mbox{\ooalign{integer}}/\mbox{\ooalign{float}}/\mbox{\ooalign{char}}\\
%Does it have multiple types?\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\

%Is it labeled data?\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}
%\end{mybox}

\begin{mybox} {Composition of the Data}
This captures information on level of homogeneity in the data.\\
a) Are the data point instances primary data type? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
b) Are all instances  similar?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
\end{mybox}

\begin{mybox} {Format of the Data}
This covers a set of sub-facets including format
The format of the file is the format in which the information in the file is stored - common
examples being csv, pdf or gif. Some formats in general have been more widely used with greater support for interoperability and processing.  In the case of structured data, the data set has a
schema if, apart from the data, there is also metadata that tells us something about the
relationship of the different data items. It is relational data if it can be presented
in tabular form or moved to a relational database. In the case of standards, it is possible to check the data set against a known set of standards and understand compliance with any of them. Compliance to standards may imply availability of generic tools and query languages to operate in the data. A proprietary format is a format that is
owned by someone or some entity; however, as long as it is open, it will not be a restriction. If the format is not known, then it is not possible to answer whether the data is
in a proprietary format or not.\\
a) What is the format of the data set file?\\
\mbox{\ooalign{csv}}/\mbox{\ooalign{pdf}}/\mbox{\ooalign{tsv}}/\mbox{\ooalign{gif,jpg}}/\mbox{\ooalign{xml}}/\mbox{\ooalign{json}}/\mbox{\ooalign{other}}\\
Score: 1 for xml, json, csv, tsv; 0 for pdf, gif, jpg, other\\
%What format are the contents?\\
b) Does it have a schema?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Score: 1 and 0 respectively, for this response, and for other binary-valued responses.\\
c) Is it an export or query result of relational data? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
d) Does it adhere to a standard?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
e) If in proprietary format, is it open? \mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
f) Is it in normalized form?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}
\end{mybox}
\begin{mybox} {Data Usage}
Data that is easier to use is preferred to data that is more complex to use. These aspects are also covered in sub-facets of format and type. However this facet is being retained because in some instances, the respondent may have a specific view on this aspect of the data.\\
a) How easy is it to utilise the data? 
~\mbox{\ooalign{Simple}}/\mbox{\ooalign{Moderate}}/\mbox{\ooalign{Difficult}}/\mbox{\ooalign{Complex}}\\
Score: 1, 0.6, 0.3, 0 respectively
%b) How easy it is to setup the data?\\
%~\mbox{\ooalign{Simple}}/\mbox{\ooalign{Moderate}}/\mbox{\ooalign{Difficult}}/\mbox{\ooalign{Very difficult}}\\
%Score: 1, 0.6, 0.3 and 0 respectively
\end{mybox}

\begin{mybox} {Data Sensitivity}
This aspect could influence the data cost significantly in terms of the added risk of exposure, and need to protect the data from breaches. However it would also increase the value of the data in terms of the improved analysis that is possible. For our purpose here, we assume that if the same task can be performed with data having sensitive information and data that does not have sensitive information, then  the latter would be preferred. While the legal aspects are covered as a separate facet, there could be additional moral and ethical issues in the dissemination of such data.\\
a) Is it free of confidential information? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
b) Is it free of personal identifiable information? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
c) Is it free of information to be retained for mandatory purposes? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}} \\
d) Is it free of revenue or financial data? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
e) Does it have Medical data/ health data? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Score: 0 and 1 respectively\\
f) Does it have protective variables? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}
Score: 0 and 1 respectively
\end{mybox}

\begin{mybox} {Statistical properties}
These properties are important intermediate steps in the path to insights from data. Hence, though they may be hard to define, we are listing them here.
a) Is it suitable for classification models? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
b) Is it suitable for linear regression models? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
c) Is it suitable for clustering models?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
d) Has it been used in ML algorithms already?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
%is the data uniformly distributed over different fields?\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
e) Was any sampling applied on the data to get this sample? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
f) Is it time-series data?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
g) Is it suitable for bivariate analysis? \mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
h) Is it suitable for multivariate analysis? \mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\

\end{mybox}

\begin{mybox} {Data Granularity}
Aggregate information is generally less useful than detailed or instance-level information. \\
a) Is it aggregate or summary information?\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Score: 0, 1
\end{mybox}


\begin{mybox} {Frequency of Use}
The current frequency of use is a rough indicator of future use or disuse of the data.\\
When was the data last used? \\
~\mbox{\ooalign{This month}}/\mbox{\ooalign{This year}}/\mbox{\ooalign{In last 5 years}}/\mbox{\ooalign{More than 5 years ago}}\\
Score: 1, 0.75, 0.5 and 0 respectively

Is there a 'known' future use? \mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}
\end{mybox}

\begin{mybox} {Data Quality}
This is one aspect of data that has been quite well-studied in terms of its impact on the data value. However, the studies have again been application-specific, where the base definitions of the terms themselves have been with reference to the application at hand. We pose the following questions categorically, to be answered as best as possible as it purports to the current definition of the data set, independent of the end application. Where the respondent is unable to provide numeric values, as may happen sometimes, we have also provided a list of values to select from.  Further it is possible that especially in this section the respondent may not may not be able to answer without a context.

a) Are all the fields complete?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}?\\
b) Is it error-free?~ \mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
c) Are there known missing instances? \mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}
Score: 0 and 1 respectively\\
d) Does it fill the missing values in an existing data set? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
e) Is it complete, with respect to the purpose it defines? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
f) Is it known to have duplicates?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Score: 0 and 1 respectively\\
g) Does it complement or supplement an existing data set?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
h) Is the data accurate?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
i) What is the precision? \\
Enter a number between 0 and 1 or select one of: ~\mbox{\ooalign{High}}/\mbox{\ooalign{Medium}}/\mbox{\ooalign{Low}}\\
j) What is the recall? \\
Enter a number between 0 and 1 or select one of: ~\mbox{\ooalign{High}}/\mbox{\ooalign{Medium}}/\mbox{\ooalign{Low}}\\
Score: Numeric value or 1,0.5 and 0 respectively\\
k) Is the data consistent within the data set? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Score: Numeric value or 1,0.5 and 0 respectively\\
l) Does the data have noise?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Score: 0 and 1 respectively
\end{mybox}






\begin{mybox} {Data Velocity}
This is the rate at which the data arrives. It influences the design of the data store systems and the plans for
scalability. Specifically for streaming it requires computational resources.\\
a) How rapidly can it be said to be generated? \\
\mbox{\ooalign{Very fast}}/\mbox{\ooalign{Fast}}/\mbox{\ooalign{Medium}}/\mbox{\ooalign{Not significant}}\\
Score: 0.5, 0.75, 1.0 and 1.0 respectively
%b) How rapidly can it be consumed?\\
%\mbox{\ooalign{Very fast}}/\mbox{\ooalign{Fast}}/\mbox{\ooalign{Medium}}/\mbox{\ooalign{Slowly}}\\
%Score: 1, 0.75, 0.5 and 0 respectively\\
b) Is it streaming data?\\
\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}} \\
\end{mybox}



\begin{mybox} {Data Sourcing}
The source of the data, including the purpose of creation of the data, again bear on the cost of generation, ease of availability in general to others, whether there are alternate sources and how straightforward or not the data collection exercise is.  Single sources poses lesser overhead in terms of maintaining updates while multiple sources require synchronization from different sources to keep the data update if one portion gets updated.
a) Can this data be easily accessed by all? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}} \\
Score: 0 and 1 respectively\\
b) How was the data obtained?
~\mbox{\ooalign{Survey}}/\mbox{\ooalign{Customer feedback}}/\mbox{\ooalign{Transactional}}/\mbox{\ooalign{Web crawler}} /\mbox{\ooalign{Licensing}}/\mbox{\ooalign{Outright purchase}}/\mbox{\ooalign{Others}}\\
Score: 1,1,0.5,0,0.5,0.75,0 respectively\\
c) Is the data aggregated from many sources or from single source?
~\mbox{\ooalign{Multiple sources}}/\mbox{\ooalign{Single source}}\\
d) Is this data easy for me to get, difficult for others? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
e) Is this enterprise-generated?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
f) Is this publicly available?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}
Score: 0 and 1 respectively.\\
%g) Is this streaming data?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
g) Is this data machine generated?~
\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}
Score: 0 and 1 respectively.\\
h) Are there known alternates for this data set?
~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}
Score: 0 and 1 respectively.
\end{mybox}

\begin{mybox} {Transformation on the data}
Transformations on the data indicate that some level of processing has already been done on the data in order to make it more consumable. Some transformations such as data anonymization may reduce the potential for some kinds of personalized analysis. However, in the absence of context, we posit that anonymized data, which can be shared more readily, is preferred to non-anonymized data.\\
Is it known to have had data transformations?\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}} \\
Is it encrypted data?\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Is it anonymized data? \mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}
\end{mybox}
\begin{mybox} {Data processing}
Presence of tools to read and analyse the data makes it more useful than otherwise.\\
a) Are there tools or programs to cleanse the data? \mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
b) Are there tools or programs to process the data in the current format? \mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}
\end{mybox}





\begin{mybox} {Enterprise aspects}
The aspects of data here determine how it is perceived in the enterprise, in a general context.\\
a) Is the data already making money? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}} \\
%b) What is the value as determined by the seller for the data?\\
%b) If creating a new application - what is revenue of the new application?\\
b) Will it improve the efficiency of an existing application or business process? \\
~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}} \\
c) Does it introduce a new channel to reach to customers?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
d) Does it complement an existing application? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
e) Does it increase customer reach?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
%f) Does it get new customers?\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
f) Which parts of the business process does it contribute to? \\
~\mbox{\ooalign{Sales}}/\mbox{\ooalign{Marketing}}/\mbox{\ooalign{HR}}/\mbox{\ooalign{Operations}}/\mbox{\ooalign{Finance}}//
/\mbox{\ooalign{Accounting}}/\mbox{\ooalign{Payroll}}/\mbox{\ooalign{Others}}\\
Score: 0 for Others and 1 for everything else\\
g) At which hierarchy in the organization is the data used?
~\mbox{\ooalign{Executive}}/\mbox{\ooalign{Middle management}}/\mbox{\ooalign{Others}}/\mbox{\ooalign{Multiple}}\\
Score: 1,0.75, 0.5 and 1 respectively
\end{mybox}






\begin{mybox} {Legal and Access Aspects}
In a manner similar to the use of sensitive data, when a data set is unconditionally available for an application, it is preferred to a data set that may have legal controls or other restrictions operating on it. Ease of access in this context implies that there are not too many procedures or processes that make it difficult to start using the data.\\
a) Is this data free of any legal restrictions in usage?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}} \\
b) Was this data acquired as part of some contract? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Score: 0 and 1 respectively\\
c) Are there any contractual obligations on the data? ~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Score: 0 and 1 respectively\\
d) If pertaining to 'information about people', was there consent to use?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}} \\
e) Is it governed by some license?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}} \\
Score: 0 and 1 respectively\\
f) Are there export restrictions?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}\\
Score: 0 and 1 respectively\\
g) Is the data easy to access?~\mbox{\ooalign{y\cr\hidewidth$\square$\hidewidth\cr}}/\mbox{\ooalign{n\cr\hidewidth$\square$\hidewidth\cr}}

\end{mybox}




%\begin{mybox} {Other Data Information}
%Image data: What is the characteristics of a this data? - higher resolution or lower resolution picture,
%\end{mybox}



==> systemoverview-part2.tex <==
%\section{Data Value under Different Scenarios}
%\label{systemOverview2}

%In Section~\ref{background} we have listed the facets across which the evaluation of a data set takes place and in Section~\ref{systemOverview1} we describe how to reach a quantification based on the responses to a set of questions. In this section we substantiate the approach we have taken as a starting step for categorical data value assessment. 

%\subsection{Data Value independent of the Application}
%\label{datavalueIndeptOfAppln}
%Equation \ref{eqn:dv} may be viewed as a multi-attribute utility model of the data value, where the different attributes are captured in the sub-facets and the weightage for each attribute may be viewed as the utility of that attribute for the person performing the assessment. 
%In multi-attribute utility theory, the utility of the various attributes is known or can be determined in some manner. 
%In the context of evaluating data, the utility is typically known only to the end-user who has an application in mind, and not necessarily to the person holding the data. Hence in this case, we take the approach that for some characteristics, there are some values that are typically preferred over others. For instance, more recent data is preferred to less recent data in general, or data without noise is preferred to data with noise. 

%Given a set of assumptions on the preferred values for various characteristics, it is then possible to arrive at a weighted sum of the preferred values. 
%In equation \ref{eqn:dv} there are two parameters that affects the data value. One is the value of a sub-facet as represented in the user's response. There are multiple ways of constructing an ordering, and as we have more information of the end-use, it will be possible to assign a better ordering for the possible values in a response. We have based the ordering on typical user preferences so that we have a way of bootstrapping and getting started. The other parameter in the equation is the relative weights of each of the sub-facets. We are assuming an extremely simple case, where the relative weights of the sub-facets, represented in the above equation by $\alpha$ may be assumed to be equal, or in other words, all the aspects are assumed to have equal utility. When we have more domain knowledge, we can refine the values of $\alpha$ also.
%which will not be the case in most scenarios. Where the relative importance of the various sub-facets are not known, at the simplest we can assume $\alpha$ is always 1, and all sub-facets are treated equally, in the absence of any additional information.
%(Note to Kala - this needs to be fixed.)

%In the following section, we will describe our analysis of over $10000$ data sets from Kaggle, to establish an ordering of the values for a characteristic. When some assessor has more specific information of the end-use, then this may be factored in to compute the $\alpha$'s
%At the end of an assessment, we can associate a data set with a number representing its value on a set of assumptions. While the number by itself may not signify much on an absolute scale, comparing the numbers for two data sets, under the same set of assumptions, now becomes possible and meaningful.

%\subsection{Data Value with respect to an Application}

%When the application or end-use is known, it is easier to describe a means of assigning a value to the data set. Since the application is known,  the ordering of values for each sub-facet can be modified as needed to match the needs of the application. Further, the relative weights of each of the sub-facets can also be determined more precisely. A hypothetical data set that meets all the needs of the application is constructed, and the maximum score that can be obtained, when all the data characteristics match with the required characteristics of the application, is computed. The score for the data set at hand is computed. A comparison of the two scores reveals how much the current data set falls short of the ideal data set for the application. Since the context is known, even those questions that are dependent on an application for a response, are now answered. 

%Let us consider the following example. An application performs a study on `prisons data' and would like to understand whether an individual coming to prison will likely exhibit recidivism (relapse into old patterns of behaviour) or not. The data set~\cite{},  is available at the aggregate level rather than at the individual level. Against this goal of identifying individuals who can exhibit recidivism, this data set is not likely to have any value as predictions have to be performed by studying individual characteristics. For a different use case like understanding which state shows the most bias towards the leniency, the same data set has significant value. Let us consider another example of a data set which has personally identifiable information (PII). This information has the potential to help marketeers perform targeted advertising.  The data value of this data set would be higher for monetizing compared to those available in the public domain and that do not have any PII. Similarly data sets that are more easily available do not present a competitive advantage in terms of information value, but may possess an advantage of typically having more tools to analyse them.


%\subsection{Data Value for comparing data sets}
%As we mention above in section~\ref{datavalueIndeptOfAppln}, characterizing a data set with a number by itself may not be an end in itself. However, when comparing two or more data sets, since the comparison is done on the same set of assumptions, this is a usable number. Hence the user can get answers to questions like, ``Given $n$ datasets, how can I rank them in order of preference, with some starting assumptions on the priority of ordering on the values?". It is in such cases  a categorical assessment of data is useful.
%Supposing we compute the data value of data sets in a data catalog platform like IBM WDP \cite{} or Kaggle \cite{}, what is the information we get about the data? Independently computed data values for each data set are useful in that they provide a quantitative basis that can be used for further comparisons. 

%The biggest benefit of having a quantitative measurement is that it forms a basis that can be used to  compare the value across data sets. For example, Given two data sets (or multiple), what is the ranking of the data sets according to the value. 
%What is the comparative  value of these data sets either in the presence of application or otherwise? These data value makes sense  only when different data sets are available and we are able to rank each of the data sets either independently or in the presence of the application. 


%We would like to answer the following question:
%\textit{`Given  many data sets, can we say which data set has more value than the other'}. This question will help buyers of the data to
%assess data value between multiple data sets that satisfy the same requirements. It also helps buyers to identify data sets having better features compared to the others, other things being equal. It will also help the holder of the data understand the trade-offs against different storage tiers, for these data sets.

%Consider the answer sheet for the questionnaire for each of the data sets. Let the answer sheet be $A_{1}.... A_{n}$, where $A_{n}$ represents the answer sheet for the $n^{th}$  questionnaire; the goal is to rank the data sets based on these answer sheets in terms of its value with respect to the other sheets.  This method can be also used to derive ranking for individual facets. The facets ranking can be completely different for each facet across the data sets.   

%In the absence of the application, the ranking can be obtained by organizing the data value in the ascending order. The data value is derived for the questions that can be answered independent of the applications. In the presence of the application the relative priorities of the facets are derived based the application and the data values are computed considering all question relevant when the application is available.


%Comparing two data sets can be made simpler where data value is computed for each of the data sets with respect to a application and ordering them in the ascending values. However, the relative weights for each of the facets with respect to each data set will be lost. 

 



%\subsection{Data Value for Assessment by Buyers and Sellers}

%A practitiner can be either a buyer or a seller of the data set. The

